Revisiting Agnostic Boosting

Boosting is a key method in statistical learning, allowing for converting weak learners into strong ones. While well studied in the realizable case, the statistical properties of weak-to-strong learning remain less understood in the agnostic setting, where there are no assumptions on the distribution of the labels. In this work, we propose a new agnostic boosting algorithm with substantially improved sample complexity compared to prior works under very general assumptions. Our approach is based on a reduction to the realizable case, followed by a margin-based filtering of high-quality hypotheses. Furthermore, we show a nearly-matching lower bound, settling the sample complexity of agnostic boosting up to logarithmic factors.

==> mathstyle.tex <==
\usepackage{bm}

\makeatletter
\newcommand{\alphacmd@factory}[1]{}
\newcounter{alphacmdcounter}
\newcommand{\GenerateAlphabetCmds}[2]{%
    \renewcommand{\alphacmd@factory}[1]{%
        \expandafter\providecommand\csname #1##1\endcsname{{#2{##1}}}%
    }
    \setcounter{alphacmdcounter}{0}
    \loop
        \stepcounter{alphacmdcounter}
        \edef\alphacmd@ID{\@Alph\c@alphacmdcounter}
        \expandafter\alphacmd@factory\alphacmd@ID
    \ifnum\thealphacmdcounter<26
    \repeat
}

\newcommand{\GenerateAlphabetCmdsLower}[2]{%
    \renewcommand{\alphacmd@factory}[1]{%
        \expandafter\providecommand\csname #1##1\endcsname{{#2{##1}}}%
    }
    \setcounter{alphacmdcounter}{0}
    \loop
        \stepcounter{alphacmdcounter}
        \edef\alphacmd@ID{\@alph\c@alphacmdcounter}
        \expandafter\alphacmd@factory\alphacmd@ID
    \ifnum\thealphacmdcounter<26
    \repeat
}
\makeatother


\GenerateAlphabetCmds{}{\mathbb}

\GenerateAlphabetCmds{c}{\mathcal}

\newcommand*{\StyleRand}[1]{\mathbf{#1}}
\GenerateAlphabetCmds{r}{\StyleRand}
\GenerateAlphabetCmdsLower{r}{\StyleRand}
\newcommand*{\ralpha}{\bm{\alpha}}
\newcommand*{\rgamma}{\bm{\gamma}}
\newcommand*{\reps}{\bm{\eps}}
\newcommand*{\rsigma}{\bm{\sigma}}


\newcommand*{\StyleDist}{\mathcal}
\GenerateAlphabetCmds{d}{\StyleDist}
\newcommand*{\StyleRandDist}[1]{\bm{\StyleDist{#1}}}
\GenerateAlphabetCmds{rd}{\StyleRandDist}

\newcommand*{\StyleSet}{\mathnormal}
\GenerateAlphabetCmds{s}{\StyleSet}
\newcommand*{\StyleRandSet}{\bm}
\GenerateAlphabetCmds{rs}{\StyleRandSet}

\newcommand*{\StyleFamily}{\mathcal}
\GenerateAlphabetCmds{f}{\StyleFamily}
\newcommand*{\StyleRandFamily}[1]{{\bm{\mathcal{#1}}}}
\GenerateAlphabetCmds{rf}{\StyleRandFamily}

\newcommand*{\StyleVec}{\vec}
\GenerateAlphabetCmdsLower{v}{\StyleVec}
\newcommand*{\vzero}{\StyleVec{0}}
\newcommand*{\StyleRandVec}[1]{\StyleRand{\StyleVec{#1}}}
\GenerateAlphabetCmdsLower{rv}{\StyleRandVec}
\newcommand*{\rvzero}{\StyleRandVec{\vzero}}

